Generating robust counterfactual explanations

Counterfactual explanations have become a mainstay of the XAI field. This particularly intuitive statement allows the user to understand what small but necessary changes would have to be made to a given situation in order to change a model prediction. The quality of a counterfactual depends on several criteria: realism, actionability, validity, robustness, etc. In this paper, we are interested in the notion of robustness of a counterfactual. More precisely, we focus on robustness to counterfactual input changes. This form of robustness is particularly challenging as it involves a trade-off between the robustness of the counterfactual and the proximity with the example to explain. We propose a new framework, CROCO, that generates robust counterfactuals while managing effectively this trade-off, and guarantees the user a minimal robustness. An empirical evaluation on tabular datasets confirms the relevance and effectiveness of our approach.

==> tables/table_area_under_curves.tex <==
\begin{table}[tb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
& & \multicolumn{2}{c}{Compas} & \multicolumn{2}{c}{GMC} \\
\cmidrule(l){2-2} \cmidrule(l){3-4} \cmidrule(l){5-6}
& Measures  &  PROB &  \CostRC &  PROB &  \CostRC  \\
\midrule
 & Area under the curve ($\downarrow$) &  $0.04$ &    $\bm{0.02}$ &    $2.49$ &    $\bm{0.01}$\\
\end{tabular}
}
\caption{Comparison between PROB and \CostRC for $\sigma^2=0.01$. For each of the two methods, we compute the area under the curve presented in Figures \ref{fig:trade_off_compas} and \ref{fig:trade_off_give_me_credit}.}
\label{table:comparision_areas}
\end{table}

==> tables/table_results.tex <==
\begin{table}[tb]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccc}
\toprule
& & \multicolumn{4}{c}{Adult} & \multicolumn{4}{c}{Compas} & \multicolumn{4}{c}{GMC} \\
\cmidrule(l){2-2} \cmidrule(l){3-6} \cmidrule(l){7-10} \cmidrule(l){11-14}
& Measures  &  $PROB_{0.15}$ &  $\CostRC_{0.15}$ &  $PROB_{0.35}$ &  $\CostRC_{0.35}$ & $PROB_{0.15}$ & $\CostRC_{0.15}$ &  $PROB_{0.35}$ &  $\CostRC_{0.35}$  &  $PROB_{0.15}$ &       $\CostRC_{0.15}$ &  $PROB_{0.35}$ &  $\CostRC_{0.35}$ \\
\midrule
& Validity ($\downarrow$) &   $\bm{1.0}$ &   $\bm{1.0}$ &   $\bm{1.0}$ &   $\bm{1.0}$ &   $\bm{1.0}$ &   $\bm{1.0}$ &  $\bm{1.0}$ &  $\bm{1.0}$ &  $\bm{1.0}$ &  $\bm{1.0}$ &  $\bm{1.0}$ &  $\bm{1.0}$\\
& Robustness ($\uparrow$) &  $\bm{0.19 \pm 0.04}$ &    
$0.22 \pm 0.02$ &    $0.36 \pm 0.01$ &    $\bm{0.29 \pm 0.02}$ &    $\bm{0.13 \pm 0.02}$ & $0.15\pm 0.03$ & $0.33 \pm 0.02$ & $\bm{0.24 \pm 0.03}$ & $\bm{0.14\pm0.02}$ & $0.17\pm0.02$ & $0.30\pm 0.03$ & $ \bm{0.22\pm0.02}$ \\
& Proximity ($\downarrow$) &   $6.24 \pm 6.75$ &  $\bm{0.19 \pm 0.05}$ &  $1.07 \pm 1.57$ &  $\bm{0.16 \pm 0.05}$ & $0.34 \pm 0.15$ & $\bm{0.28\pm 0.11}$ & $\bm{0.21\pm0.12}$ & $0.22 \pm 0.10$ & $1.38\pm3.01$ & $\bm{0.14 \pm 0.04}$ & $\bm{0.11\pm0.05}$ & $0.12\pm0.03$  \\
 
\end{tabular}
}
\caption{Comparison between PROB and \CostRC for $\sigma^2=0.01$ and for a target of $0.15$ and $0.35$.}
\label{table:comparision_results}
\end{table}
